GCRayDiffusion: Pose-Free Surface Reconstruction via Geometric Consistent Ray Diffusion

Accurate surface reconstruction from unposed images is crucial for efficient 3D object or scene creation. However, it remains challenging, particularly for the joint camera pose estimation. Previous approaches have achieved impressive pose-free surface reconstruction results in dense-view settings, but could easily fail for sparse-view scenarios without sufficient visual overlap. In this paper, we propose a new technique for pose-free surface reconstruction, which follows triplane-based signed distance field (SDF) learning but regularizes the learning by explicit points sampled from ray-based diffusion of camera pose estimation. Our key contribution is a novel Geometric Consistent Ray Diffusion model (GCRayDiffusion), where we represent camera poses as neural bundle rays and regress the distribution of noisy rays via a diffusion model. More importantly, we further condition the denoising process of RGRayDiffusion using the triplane-based SDF of the entire scene, which provides effective 3D consistent regularization to achieve multi-view consistent camera pose estimation. Finally, we incorporate RGRayDiffusion into the triplane-based SDF learning by introducing on-surface geometric regularization from the sampling points of the neural bundle rays, which leads to highly accurate pose-free surface reconstruction results even for sparse-view inputs. Extensive evaluations on public datasets show that our GCRayDiffusion achieves more accurate camera pose estimation than previous approaches, with geometrically more consistent surface reconstruction results, especially given sparse-view inputs.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.

\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/result/dust3r_case1.png} \\
        \includegraphics[width=\linewidth]{image2.png} \\
        \includegraphics[width=\linewidth]{image3.png} \\
        \includegraphics[width=\linewidth]{image4.png}
        \caption{Images}
    \end{minipage} \hfill
    \begin{minipage}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pose_diffusion_1.png} \\
        \includegraphics[width=\linewidth]{pose_diffusion_2.png} \\
        \includegraphics[width=\linewidth]{pose_diffusion_3.png} \\
        \includegraphics[width=\linewidth]{pose_diffusion_4.png}
        \caption{Pose Diffusion}
    \end{minipage} \hfill
    \begin{minipage}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{relpose_1.png} \\
        \includegraphics[width=\linewidth]{relpose_2.png} \\
        \includegraphics[width=\linewidth]{relpose_3.png} \\
        \includegraphics[width=\linewidth]{relpose_4.png}
        \caption{RelPose++}
    \end{minipage} \hfill
    \begin{minipage}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ray_regression_1.png} \\
        \includegraphics[width=\linewidth]{ray_regression_2.png} \\
        \includegraphics[width=\linewidth]{ray_regression_3.png} \\
        \includegraphics[width=\linewidth]{ray_regression_4.png}
        \caption{Ray Regression (Ours)}
    \end{minipage} \hfill
    \begin{minipage}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ray_diffusion_1.png} \\
        \includegraphics[width=\linewidth]{ray_diffusion_2.png} \\
        \includegraphics[width=\linewidth]{ray_diffusion_3.png} \\
        \includegraphics[width=\linewidth]{ray_diffusion_4.png}
        \caption{Ray Diffusion (Ours)}
    \end{minipage}
\end{figure}


%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/5_sup.tex <==
\newpage

\section{More Details of Camera Estimation from Neural Ray Bundles}

Given a collection of neural bundle rays $\mathcal{R}_i$ associated with 2D pixels $\{u_k\}_{M}$, here we can give the derivation details to recover the camera pose $T$ by solving the intersection of all rays in $\mathcal{R}_i$.

Specifically, we begin by defining each ray in the bundle that each ray $\textbf{r}_k^i$ is represented as a 7-dimension vector including a unit directional vector $\textbf{v}^i_k \in R^3$ through any point $\textbf{p}^i_k \in R^3$ and depth $d^i_k \in R$ following Pl$\ddot{u}$cker coordinates~\cite{Plucker1828} as:
\begin{equation}
    \textbf{r}_k^i = (\textbf{v}^i_k , \textbf{m}^i_k , \textbf{d}^i_k) \in R^7,
\end{equation}

 For each ray, we have the corresponding 2D pixel $u_k$ in the image plane, which we can relate to the 3D scene via the camera's intrinsic and extrinsic parameters.

Next, we aim to recover the camera's pose, represented by a transformation matrix $T$. This matrix consists of the rotation and translation of the camera, mapping 3D world coordinates to 2D image coordinates. We solve for the camera pose by finding the intersection of the rays in the bundle $\mathcal{R}_i$. In practice, this involves solving the system of equations resulting from the projection of the 3D rays onto the 2D image plane, using the camera's intrinsic parameters.

Let the projection matrix $P$ be defined as:
\[
P = K [R | t]
\]
where $K$ is the intrinsic matrix of the camera, $R$ is the rotation matrix, and $t$ is the translation vector. The goal is to estimate $R$ and $t$ such that the projected rays from the world coordinates align with the observed rays in the image. This is achieved by minimizing the geometric error between the projected 3D points and the corresponding 2D points.

To perform this optimization, we can use methods such as bundle adjustment or direct least squares optimization, which iteratively adjusts $R$ and $t$ to minimize the projection error across all rays in $\mathcal{R}_i$. The solution is the camera pose $T$ that best explains the observed rays.

Once the camera pose is recovered, we can refine it by considering the depth information from the rays and adjusting the parameters to improve the alignment of the rays with the 3D scene. This approach provides a robust way to estimate camera poses from neural ray bundles, leveraging the geometry of the rays and the 3D structure captured in the scene.

\section{More Details on Experiments}

\textbf{More Details of Image Feature Extractor $F_{\mathcal{I}}$.} We use the DINOV2 transformer-based image encoder for feature extraction. 

The image encoder is responsible for extracting the feature maps from the image input, which are then processed further by the downstream models.

\textbf{More Details of Triplane-based SDF $F_{\theta}$.} We formulate $F_{\theta}$ as a triplane-based signed distance field (SDF), which consists of a Transformer-based image encoder ${\varPhi}$ to extract triplane feature maps from image inputs and a MLP-based decoder $\mathcal{D}$ to regress the SDF prediction. 

The triplane's initial size is $32 \times 32$ with $512$ output channels. After up-sampling, a Multihead MLP (Multilayer Perceptron) is used to decode the Signed Distance Function (SDF). The up-sampling operation increases the spatial resolution, while the Multihead MLP helps to refine the feature map and interpret the SDF, allowing the model to better capture the underlying geometry and surface details. 

\textbf{Time and Efficiency Analysis.} Here we give more details of our GCRayDiffusion in terms of inference time and GPU memory storage for each main components, including the image feature extraction (IFE), geometric consistent ray diffuser (GCRD) and triplane-based SDF (SDF) respectively.

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
         & IFE & GCRD & SDF \\ \hline
        Time   & 50ms   & 200ms   & 300ms  \\ 
        GPU Storage   & 1G   & 1G   & 2G   \\ \hline
    \end{tabular}
    \caption{The inference time for each component of our GCRayDiffusion}
    \label{tab:1}
\end{table}

As shown in Table~\ref{tab:1}, on average the IFE module takes about 50ms for image feature extraction, GCRD takes about 200ms and SDF takes about 300ms for ray diffuser and SDF learning respectively. As for the GPU memory storage, on average IFE module costs about 1G for image feature extraction, GCRD costs about 1G and SDF cost about 3G for ray diffuser and SDF learning respectively.

\textbf{More Visual Comparison Results.} Fig.~\ref{fig: sup comparison1} to Fig.~\ref{fig: sup comparison4} show more visual surface reconstruction and camera pose estimation results evaluated on Objaverse and GSO dataset for different comparing approaches, including RelPose++, FORGE, DUSt3R and our GCRayDiffusion rescptively.

\section{Limitation and Discussion}
One main limitation of our current solution in GCRayDiffusion is that the geometric consistent ray diffuser is mainly pre-trained on single object dataset, i.e., Objaverse, therefore our GCRayDiffusion couldn't achieve satisfied camera pose estimation and surface reconstruction results for the scene scenario. One possible solution is to use large scene dataset to train our GCRayDiffusion, but there still remains challenge for scene data annotation. Moreover, it is also a challenging problem to the joint learning of camera pose estimation and surface reconstruction for large scene images, especially given sparse image input. The second limitation comes from the neural surface learning, since our current triplane-based SDF learning would also fail for extremely sparse inputs. One interesting future work is formulating both the camera pose estimation and neural surface learning as a unit diffusion processing, thus enabling very robust camera pose estimation and surface reconstruction through the diffusion even in extreme sparse inputs.    


\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{ICCV2025-Author-Kit-Feb/images/sup/sup1.png}
    \caption{Qualitative surface reconstruction comparison evaluated on Objaverse dataset for different comparing approaches, including RelPose++, FORGE, DUSt3R and our GCRayDiffusion (from left to right column) respectively.}  
    \label{fig: sup comparison1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{ICCV2025-Author-Kit-Feb/images/sup/sup2.png}
    \caption{Qualitative surface reconstruction comparison evaluated on Objaverse dataset for different comparing approaches, including RelPose++, FORGE, DUSt3R and our GCRayDiffusion (from left to right column) respectively.}  
    \label{fig: sup comparison2}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{ICCV2025-Author-Kit-Feb/images/sup/sup3.png}
    \caption{Qualitative surface reconstruction comparison evaluated on Objaverse dataset for different comparing approaches, including RelPose++, FORGE, DUSt3R and our GCRayDiffusion (from left to right column) respectively.}  
    \label{fig: sup comparison3}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{ICCV2025-Author-Kit-Feb/images/sup/3.png}
    \caption{Qualitative surface reconstruction comparison evaluated on GSO dataset for different comparing approaches, including RelPose++, FORGE, DUSt3R and our GCRayDiffusion (from left to right column) respectively.}  
    \label{fig: sup comparison4}
\end{figure*}

